Generating and Aligning from Data Geometries with Generative Adversarial Networks

Unsupervised domain mapping has attracted substantial attention in recent years due to the success of models based on the cycle-consistency assumption. These models map between two domains by fooling a probabilistic discriminator, thereby matching the probability distributions of the real and generated data. Instead of this probabilistic approach, we cast the problem in terms of aligning the geometry of the manifolds of the two domains. We introduce the Manifold Geometry Matching Generative Adversarial Network (MGM GAN), which adds two novel mechanisms to facilitate GANs sampling from the geometry of the manifold rather than the density and then aligning two manifold geometries: (1) an importance sampling technique that reweights points based on their density on the manifold, making the discriminator only able to discern geometry and (2) a penalty adapted from traditional manifold alignment literature that explicitly enforces the geometry to be preserved. The MGM GAN leverages the manifolds arising from a pre-trained autoencoder to bridge the gap between formal manifold alignment literature and existing GAN work, and demonstrate the advantages of modeling the manifold geometry over its density.

==> introduction_old.tex <==
In many important settings for generative deep learning models, from images to biology, we wish to generate complex high-dimensional data that lies on a simpler, low-dimensional manifold. In recent years, the success of generative adversarial networks (GANs) at modeling such high-dimensional data has prompted their use in many such settings~\cite{zhu2016generative,huang2017manifold}. One application that has received considerable interest arises when there is not one data distribution but two, and we wish to map between them~\cite{isola2017image}. Examples include having two sets of images with different styles or subjects, having a text corpus (e.g. captions) and a related set of images they describe, and having measurements from a biological experiment on two different individuals~\cite{zhu2017unpaired,zhang2018translating,hosseini2018multi,amodio2018magan}.

The goal in common to each of these cases is that of unsupervised domain mapping: we have samples from two data distributions and wish to map between them, but we do not have any information labeling a point in one domain with its respective representation in the other domain. The earliest methods for domain mapping required supervision~\cite{isola2017image,van2015transfer}, while unsupervised domain mapping came to the forefront with the introduction of cycle-consistent GANs~\cite{zhu2017unpaired,kim2017learning}. Cycle-consistent GANs simultaneously learn two generative functions: one that maps from the first dataset to the second dataset and vice versa. Many such pairs of generative functions exist, however, so the key assumption constraining these architectures is that the two generative functions should be each other's inverse. In other words, mapping a point from the first domain to the second with a generator and then applying the other generator to this new second domain point should yield the original point in the first domain. In practice, cycle-consistent GANs have achieved impressive results on a wide range of applications~\cite{hoffman2017cycada,zhu2017unpaired,chu2017cyclegan}.

% Procrustes alignment~\cite{luo2002procrustes}

In this paper we cast the problem of unsupervised domain mapping as one of manifold alignment between the two domains. While previous work on unsupervised domain mapping has implicitly invoked manifold alignment terminology, no concrete approach from the manifold literature is introduced~\cite{brunner2018symbolic,wang2018generating,zhu2018emotion,chen2018cartoongan}. In fact, in this manuscript, we show that cycle-consistent GANs on their own are inappropriate for manifold alignment for two reasons (shown in Figure~\ref{fig:cartoon1}), and introduce a novel framework to address these problems.

First, the discriminators force the generators to match the target data distribution probabilistically, rather than geometrically (Figure~\ref{fig:cartoon1}a). This is because of the probabilistic prediction in the minimax game that the generator and discriminator are playing. The discriminator does not try to predict whether a given point \textit{could} be real, but instead tries to predict whether a given point \textit{is more likely} to be real or fake. The most obvious illustration of the problem with this approach is if our two datasets are different samples from the same underlying distribution. The cycle-consistent GANs will change points when going from domain to domain to reflect the sampling error, rather than learning the identity function as it should because they lie on the same manifold. In fact, the identity function is not even an optimum to either the generator or discriminator loss in this case, as it leaves some areas of the space more likely to be in one domain or the other.

Second, in cycle-consistent GANs, the representation of a point in the source domain is not tied to its representation in the target domain in any way (Figure~\ref{fig:cartoon1}b). The generators are required to be inverses of each other, but the generator is allowed to make any arbitrary invertible change to the data: even if it does not preserve the manifold geometry. Consequently, while the generator does learn to sample from the target distribution when given data from the source distribution, it is inappropriate to describe these GANs as performing \textit{manifold alignment}.

We introduce a new model to remedy these problems by bringing concepts from manifold alignment~\cite{tenenbaum2000global,wang2013manifold} and statistical sampling~\cite{neal2001annealed} and incorporating them in the cycle-consistent GAN framework. Our model thus truly aligns two data manifolds in an unsupervised way. To emphasize the difference, we call our model the \textit{Manifold Geometry Matching GAN}, or MGM GAN.

The MGM GAN leverages the latent space of a third network, a pre-trained autoencoder, to obtain a representation of the manifold for each dataset, as autoencoders have been demonstrated to be effective at this learning both in theory and practice~\cite{vincent2010stacked,vincent2008extracting,holden2015learning,bengio2013representation,goodfellow2016deep}. Since the manifold is then entirely parameterized by a neural network, it is differentiable and can be used to train the generator. With this manifold, we introduce two novel additions to the MGM GAN that facilitate manifold alignment:
\begin{enumerate}
    \item an importance sampling technique which calculates weights for each point based on a Voronoi partition of the manifold to offset differences in density between the domains in each partition
    \item a manifold geometry loss adapted from formal manifold alignment literature
\end{enumerate}

By explicitly minimizing the manifold geometry loss, the generators are encouraged to align the manifolds as best as they can without distorting the original points unnecessarily. By weighting each point inversely to the density in its region of the manifold, we make the density along the manifold constant and prevent the discriminator from picking up on any differences in density.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/cartoon1-01.png}
    \caption{Two examples of a GAN not aligning data manifolds when underlying populations are sampled at different frequencies in the two domains. (a) The traditional GAN loss forces density to be matched rather than geometry. (b) The generator can sever the manifold geometry, mapping two similar points to two very different targets or two different points to two very similar targets.}
    \label{fig:cartoon1}
\end{figure}



\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/cartoon2-01.png}
    \caption{The MGM GAN architecture first extracts the latent representations of the data from an autoencoder to approximate the data manifold. Then, (a) our importance sampling scheme balances the densities along the manifold and (b) a manifold geometry loss preserves the relationships between points on the manifold after mapping to the other domain.}
    \label{fig:cartoon2}
\end{figure*}

In addition to matching manifold geometry, the introduction of these novel losses addresses a key problem in cycle-consistent GANs: model ambiguity. Previous work has shown that cycle-consistent GANs can learn a great variety of different mappings that all fool the discriminator at the distribution level~\cite{amodio2018magan,dumoulin2016adversarially,perera2018in2i,li2017alice}. However, these do not necessarily yield alignment between individual source and target points, i.e. it may shuffle the arrangement of points as it transforms the manifold. In the MGM GAN, the manifold geometry loss resolves the ambiguity by explicitly forcing the arrangement of points on the manifold to be preserved as best as possible.

In the rest of this paper, we first formally describe the MGM GAN framework. Then, we describe several applications where manifold alignment, rather than data distribution alignment, is more desirable. We show that previous GANs change the data far more than necessary because they match data distributions and not manifolds, while the MGM GAN truly aligns manifolds. We demonstrate this on simulated data, image data from the canonical MNIST dataset, and biological data.




